The Vanishing Decision Boundary Complexity and the Strong First Component

We show that unlike machine learning classifiers, there are no complex boundary structures in the decision boundaries for well-trained deep models. However, we found that the complicated structures do appear in training but they vanish shortly after shaping. This is a pessimistic news if one seeks to capture different levels of complexity in the decision boundary for understanding generalization, which works well in machine learning. Nonetheless, we found that the decision boundaries of predecessor models on the training data are reflective of the final model's generalization. We show how to use the predecessor decision boundaries for studying the generalization of deep models. We have three major findings. One is on the strength of the first principle component of deep models, another about the singularity of optimizers, and the other on the effects of the skip connections in ResNets. Code is at https://github.com/hengshu1/decision_boundary_github.

==> 0conv_pushback.tex <==

% \section{Decision Boundary Behaviors}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{db_conv_run3.png}
\caption{
Class centers changing over time. Model: VGG19. Optimizer: SGD-anneal-lr. Finally the CAT and DOG centers converge to a small neighborhood. In general, the centers have a trend of moving away from each other with some winding back (knot-like patterns). The CAT and DOG centers are taken at the same moment over the PCA(2) features on the training samples. They are symmetric to each other respect to the origin at the same moment (shown by the dashed lines). Both CAT and DOG centers are close to zero at the beginning of training. 
Most strikingly, this figure shows that the first principle component grows stronger and stronger. In fact, the second component phases out over time after the initial growth stage. The first component (out of 512 features) is strong enough to support the classification. The snapshot on the left shows the center changes in the beginning stage. The right snapshot shows the evolution of the class center in 200 epochs of training. 
}\label{fig:db_convergence}
\end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{db_conv_vgg_adam_run1.png}
% \caption{
% VGG, Adam. The class centers still changes dramatically in the end, which does not seem to have a convergence. 
% It's interesting to investigate whether this is related to the poorer generalization of Adam. 
% }\label{fig:db_convergence_vgg_adam}
% \end{figure}



% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{db_conv_run3_200epochs.png}
% \caption{
% Evolution of the principle components.
% Model: VGG19. Optimizer: SGD-anneal-lr.   
% The feature matrix is unnormalized. So this is the truncated SVD with 10 components.
% }\label{fig:db_convergence_svd_200epochs}
% \end{figure}





% In this section, we show that there are two interesting behaviors of the decision boundary during the evolution process. 
\section{Decision Boundary Convergence}
[give some figure in the appendix]
Decisions stabilize as deep models are trained with more and more data and epochs. It makes sense for the decision boundary to have a convergence behavior. However, from Figure \ref{fig:boundary_vanishing_pca_5}, the decision boundary did not seem to have a convergence behavior due to some accidental noise. In our initial experiments, the cats and dogs can even switch from one side to the other side of the $y$-axis for some of the predecessor models shown. 

A careful examination of the plots shows that except the sign changing, the centers of cats and dogs across the plotted moments do have a trend of moving away from each other. That the cats and dogs switching side is merely an accidental noise by the PCA procedure, which returns the components with a random sign. The sign of the principle components does not matter in most applications of PCA. However, it matters in our context because we are studying the evolution of the principle components over time.  To account for a stable sign for the components over time, we make sure the CAT center is always on the left side of the DOG center. This is done by detecting whether the reverse happens and if so their positions are switched.  

Figure \ref{fig:db_convergence} shows the plot of the centers of CAT and DOG over time, calculated from the mean of all the training samples per class in the PCA(2) space. The moments shows from the beginning of training all the way to the final model. Moments are sampled near every 5\% increase in the training accuracy with the last few moments for models achieving over 99\% training accuracy. The plot has an interesting pattern: The CAT center and DOG center symmetrically moves away from each other over time. Note because the mean of a principle component (over all samples including cats and dogs) is zero, the mean of the CAT center and DOG center is also zero. Thus at all moments, the CAT and DOG centers are always symmetric with respect to the origin. Interesting, the overall movements look like they are all centered around the center(s) from the initial model. This is also true because for the initial model, the CAT and DOG centers are both very close to the origin (because the two classes are not splitted yet). 
The last five points in the trajectory correspond to the center from the predecessor models near the end, 99.48\%, 99.84\%, 99.87\%, 99.97\% and 100\%. It is clear that both the CAT and DOG centers finally converge to a small neighborhood. 



If we look at the magnitudes of the components, especially their changes over time, the second component shrinks and eventually closes to zero (just  where it started from). This shows in the end, the classifier is supported by only the first component. We found this ``strong'' first component phenomenon very interesting, because it is calculated from running PCA over 512 features. Reducing hundreds features down to only one and still maintains 100\% training accuracy seems bizarre for machine learning classifiers. For the 100\% training accuracy remark, check Figure \ref{fig:boundary_vanishing_pca_5} for the final decision boundary (the first plot), in which a cut vertical to the $x$-axis (first principle) near the boundary delivers it.    


% \subsection{The Push-Pushback Behavior}

% The class center evolution in the PCA space shown in Figure \ref{fig:db_convergence} is good for us to understand how the principle components change over time. Principle components are important anyway. 
% However, because of normalization in the feature matrix (input of the PCA procedure), the original features in the low-dimensional space are changed. Thus it loses track of the original feature evolution.  

% To bring this perspective back, we perform truncated SVD with the top two low-rank features. This is equivalent to PCA(2) except that the features are not normalized.   
% Figure \ref{fig:db_convergence_svd} shows the evolution of the centers in the SVD(2) space. This figure shows the beginning of training starts with lots of ``quasi-parallel'' movements in the two centers. 
% The movement lasts a long time  in the training (all the way before 90\%), e.g., see 50\% to 55\%, 75\% to 80\%, and 80\% to 85\%. However, after this stage, the two centers start moving in the opposite directions in the first feature dimension ($x$-axis), e.g., see 90\% to 95\%, and 95\% to 99.48\%. 
% The quasi-parallel movement can come back at this stage too, e.g., from the 99.84\%-model to 99.87\%-model.  


% Cat and Dog recall rates up and low shows that the boundary moving back and forth between them. Can we show this?


% capture the mean of the training cats in the first principle component. This component is computed by running PCA with two components between the boundary with DOG. 
% Also show ten typical epochs where the boundary is pushed back and forth between CAT and DOG. 
 


% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{db_conv_run3_svd.png}
% \caption{
% Class center evolution in the SVD(2) space. The evolution starts from the origin, where the CAT and DOG centers meet. 
% Model: VGG19. Optimizer: SGD-anneal-lr. The bold arrows and fonts correspond to the DOG center evolution. The ordinary arrows and fonts are the CAT center evolution. The color changes every five intervals to facilitate examination. 
% }\label{fig:db_convergence_svd}
% \end{figure}

==> 0resistors.tex <==

\section{The Resistors in Training }\label{se:resistors}
So far we have plotted all the samples of classes in the training set. It is helpful to have a closer look at the boundary area. To do this, we extract the subset of samples that are near the boundary. We explored 
For the same optimizer and model, across runs are the resistors largely the same?


\begin{figure*}[t]
\centering
\includegraphics[width=2\columnwidth]{resistors_boundary.png}
\caption{
Training resistors: 250 (5\% of the class) samples that are closest to the other class center in the 2D principle-component space. The green lines are illustration of overfit models given the features.
What is particularly interesting is, {\em the training finally did not end up with these green decision boundaries or anything alike}. Instead, the final model has super clean decision boundaries, e.g., the CAT-DOG shown in the first plot of Figure \ref{fig:boundary_vanishing_pca}. For these overfit boundaries, CAT-DOG is rather complex, especially worth noting that {\em some cats/dogs reach far inside the regions of DOG/CAT}. CAT-FROG and CAR-TRUCK are much simpler but there are still non-convex curvatures in their boundaries. 
Model: VGG19 using the 99.45\% predecessor model (same as Figure \ref{fig:boundary_cats_and_others} and Figure \ref{fig:boundary_tripple}). 
}\label{fig:boundary_closer}
\end{figure*}


The intuition of why this method works is that class pairs form their decision boundaries with different ease and training efforts. In addition, the decision boundaries of different class pairs vanish at different rates. This can be observed from Figure \ref{fig:boundary_cats_and_others}. All the plots used the same model at one epoch, and yet some class pairs had already been clearly separated, while others were still carving the decision boundary like CAT-DOG and CAT-FROG. Note that the training was near the end for the plots and the learning rate at this moment was already very small due to the use of annealing. This also indicates that classes that heavily interferes each other needs a very {\em fine carving} of their decision boundaries, requiring very small learning rates. This is also intuitive because CAT-DOG, and CAT-DOG have samples with very fine difference in appearance for this data set. 

 in Euclidean distance
 
The fact that these samples are the last to cross the decision boundary means that they are {\em training resistant}. 

We had lots of questions regarding the resistors. The following questions are particular interesting. 
\begin{itemize}

\item First and foremost, are the resistors model and optimizer dependent or independent? This is important because if they are dependent on the model or optimizer, it means training resistance is algorithm dependent; otherwise it is a property of some training samples. 

\item Are resistors good or bad? Are they beneficial to generalization or not?


\item 
Do the resistors oscillate in their label predictions in later training? Plot the Prob(CAT) and Prob(DOG) for cat resistors throughout the training. Note resistors are different for different class pairs. For example, CAT resistors are different you run PCA over CAT-DOG and CAT-FROG. This may not be good. I think we can compute those cats whose label predictions are the slowest to get close to the small region of prob(CAT)=1.0. Do some study of this. In one sentence, we should answer question 1 first. 

\item How long does each resistors remain in the boundary area?

\item Are those stubborn resistors (samples that are far behind the decision boundary on the other side) outliers?

\item What do the training resistors look like?

\item What if we remove those sample and retraining again?



\end{itemize}
 


==> icml_version/main_icml_old <==
%%%%%%%% ICML 2021 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%

%\documentclass{article}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2021} with \usepackage[nohyperref]{icml2021} above.
\usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
\usepackage{icml2021}

% If accepted, instead use the following line for the camera-ready submission:
%\usepackage[accepted]{icml2021}

% The \icmltitle you define below is probably too long as a header.
% Therefore, a short form for the running title is supplied here:
\icmltitlerunning{The Vanishing Decision Boundary and Training Resistors}

\begin{document}

\twocolumn[
\icmltitle{The Vanishing Decision Boundary and Training Resistors
% \icmltitle{The Vanishing Decision Boundary in Deep Learning
% \icmltitle{The Vanishing Decision Boundary and Minima Sharpness% in Deep Learning
%:\\
%Connecting Minima Sharpness and Boundary Structures
}
% \icmltitle{Decision Boundary Frontiers}
% \icmltitle{Understanding Class Interference of Deep Networks with Decision Boundary}

% It is OKAY to include author information, even for blind
% submissions: the style file will automatically remove it for you
% unless you've provided the [accepted] option to the icml2021
% package.

% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Country
% Industry affiliations should list Company, City, Region, Country

% You can specify symbols, otherwise they are numbered in order.
% Ideally, you should not use this facility. Affiliations will be numbered
% in order of appearance and this is the preferred way.
\icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Aeiau Zzzz}{equal,to}
\icmlauthor{Bauiu C.~Yyyy}{equal,to,goo}
\icmlauthor{Cieua Vvvvv}{goo}
\icmlauthor{Iaesut Saoeu}{ed}
\end{icmlauthorlist}

\icmlaffiliation{to}{Department of Computation, University of Torontoland, Torontoland, Canada}
\icmlaffiliation{goo}{Googol ShallowMind, New London, Michigan, USA}
\icmlaffiliation{ed}{School of Computation, University of Edenborrow, Edenborrow, United Kingdom}

\icmlcorrespondingauthor{Cieua Vvvvv}{c.vvvvv@googol.com}
\icmlcorrespondingauthor{Eee Pppp}{ep@eden.co.uk}

% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{Machine Learning, ICML}

\vskip 0.3in
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

%\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
\printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.

\input{abstract}

\input{introduction}

\input{db_evolve}

\input{resistors}

\input{related}

\input{conclusion}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DELETE THIS PART. DO NOT PLACE CONTENT AFTER THE REFERENCES!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \appendix
% \section{Do \emph{not} have an appendix here}

% \textbf{\emph{Do not put content after the references.}}
% %
% Put anything that you might normally include after the references in a separate
% supplementary file.

% We recommend that you build supplementary material in a separate document.
% If you must create one PDF and cut it up, please be careful to use a tool that
% doesn't alter the margins, and that doesn't aggressively rewrite the PDF file.
% pdftk usually works fine. 

% \textbf{Please do not use Apple's preview to cut off supplementary material.} In
% previous years it has altered margins, and created headaches at the camera-ready
% stage. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\bibliography{main}
\bibliographystyle{icml2021}

\end{document}


% This document was modified from the file originally made available by
% Pat Langley and Andrea Danyluk for ICML-2K. This version was created
% by Iain Murray in 2018, and modified by Alexandre Bouchard in
% 2019 and 2021. Previous contributors include Dan Roy, Lise Getoor and Tobias
% Scheffer, which was slightly modified from the 2010 version by
% Thorsten Joachims & Johannes Fuernkranz, slightly modified from the
% 2009 version by Kiri Wagstaff and Sam Roweis's 2008 version, which is
% slightly modified from Prasad Tadepalli's 2007 version which is a
% lightly changed version of the previous year's version by Andrew
% Moore, which was in turn edited from those of Kristian Kersting and
% Codrina Lauth. Alex Smola contributed to the algorithmic style files.

